Pretraining De-Biased Language Model with Large-scale Click Logs for Document Ranking

Pre-trained language models have achieved great success in various large-scale information retrieval tasks. However, most of pretraining tasks are based on counterfeit retrieval data where the query produced by the tailored rule is assumed as the user's issued query on the given document or passage. Therefore, we explore to use large-scale click logs to pretrain a language model instead of replying on the simulated queries. Specifically, we propose to use user behavior features to pretrain a debiased language model for document ranking. Extensive experiments on Baidu desensitization click logs validate the effectiveness of our method. Our team on WSDM Cup 2023 Pre-training for Web Search won the 1st place with a Discounted Cumulative Gain @ 10 (DCG@10) score of 12.16525 on the final leaderboard.

==> sections/acknowledgements.tex <==
%\vspace{-2mm}
\section*{Acknowledgements}
\label{acknowledgements}
\vspace{-1mm}
%This work is supported by the National Key Research and Development Program of China (2018YFC0831700), Natural Science Foundation of China (Grant No. 61732008, 61532011, 61902209, U2001212), Beijing Academy of Artificial Intelligence (BAAI) and Tsinghua University Guoqiang Research Institute.
This work is supported by the Natural Science Foundation of China (Grant No. 61732008, 61902209, U2001212), Beijing Academy of Artificial Intelligence (BAAI) and Tsinghua University Guoqiang Research Institute.
This project is also supported by Beijing Outstanding Young Scientist Program (No. BJJWZYJH012019100020098) and Intelligent Social Governance Platform, Major Innovation \& Planning Interdisciplinary Platform for the "Double-First Class" Initiative, Renmin University of China.
\vspace{-1mm}


==> sections/conclusion.tex <==
% !TEX root =  ../wsdm2022-fp-xiangsheng.tex


\section{Limitations}
\label{limit_section}
Despite we find our CNIR pipeline is effective to boost the ranking performance, we admit some limitations of our work and share some directions for the future work.

\textbf{Reranking vs first stage retrieval}: Our experiments are conducted in a reranking setting rather than first stage retrieval. Previous studies showed automatic query reformulation benefits in improving recall in the first stage retrieval~\cite{abdul2004umass}, but it is not validated in our experiments. The limited improvements when applying on BM25 in Table~\ref{qr_baseline} may also be because rule-based query reformulation is more effective in the first stage retrieval rather than the reranking scenario. 
Although we do not have experiments in the first stage retrieval, it does not mean that our CNIR pipeline is not effective in the first stage retrieval. In the future, we aim to incorporate embedding retrieval models~\cite{huang2020embedding} to further improve the first stage retrieval performance.


\textbf{Query anchoring vs query rewriting}: As discussed in Section~\ref{related work}, query reformulation is categorized into query anchoring and query rewriting. In our experiments, we only focus on query anchoring. Ideally, a good reformulated query that represents users' information needs clearly should not be limited with the original query terms. Therefore, using query rewriting technique remains to be investigated in our framework. The key challenge is to balance the tradeoff  between identifying the useless words or mistake words and misjudging the keywords in the original query.


%\vspace{-1mm}
\section{Conclusion}
\label{conclusion}
This paper presents a cooperative neural information retrieval pipeline (CNIR) with knowledge enhanced automatic query reformulation.
Different from traditional neural information retrieval framework, our pipeline sequentially reformulates a query first and then submits the reformulated query to neural retrieval models. 
%The proposed pipeline is optimized by the cooperative learning of automatic query reformulation and neural retrieval model.
Automatic query reformulation, which is designed by reinforcement learning, learns to reformulate a query according to the ranking results from neural retrieval models.
The reformulated query can better represent user information needs compared to the original query and thus be used in the training of neural retrieval models to further optimize the ranking performance.
In the proposed pipeline, we simultaneously optimize the quality of reformulated queries and ranking performance with an alternate training strategy.
Experiments show that the alternate training of both modules in CNIR are effective to improve the ranking performance and our pipeline can outperform existing retrieval model baselines.
To further improve the ranking performance, we incorporate knowledge information into automatic query reformulation and yield a better CNIR pipeline with better ranking performance.
We find that the quality of automatic query reformulation module decides how well the pipeline can achieve.
Further detailed analysis evaluates the effectiveness of different query reformulation strategies and time overheads in both training and testing.
We find our pipeline can improve existing retrieval models significantly while only increase negligible inference (or ranking) time, which is computationally applicable for practical ranking systems. 
Our work is a new framework to build neural retrieval models and provides a better understanding of how to use automatic query reformulation to guide the learning of neural retrieval models.


Despite we show different advantages of our CNIR pipeline, we also point out two limitations in our work, as discussed in Section~\ref{limit_section}. In the future, we aim to focus on these two challenges and build a better ranking system with the proposed framework.
  

==> sections/experiment.tex <==
% !TEX root =  ../wsdm2022-fp-xiangsheng.tex

\section{Experimental Setup}
\label{exp}
%In this section, we report the experimental settings in our framework. 

\begin{table}[!t]
	\centering
	\caption{Statistics of the datasets. $\textbf{Test}_1$ and $\textbf{Test}_2$ indicate the testing set of Tiangong-ST and Sogou-QCL, respectively.}
	%(i.e.,  ARCI, DSSM and Transformer)
	\begin{tabular}{lcccc}
		\toprule
		& \textbf{Train}  & \textbf{Valid} & $\textbf{Test}_1$  & $\textbf{Test}_2$ \\ \midrule
		\#queries 				& 344,942 & 4,888 & 2,000 & 900		\\
		\#sessions             & 143,155 & 2,000  & 2,000 & na. \\
		%\#avg. click\footnotemark[3] per query   & 3.29   & 3.36  & 3.52 \\
		\#avg. doc per query & 9.60   & 9.58  & 9.59 & 17.78\\ 
		\bottomrule             
	\end{tabular}
	\label{data_stat}
\end{table}

\footnotetext[3]{\color{black} Pseudo click drawn from PSCM labels, where documents with top 29\% click probability (grade 1 or higher) are considered being clicked.}
\addtocounter{footnote}{1}



\subsection{Dataset}
\label{data_section}
%Our experiment is conducted on a large-scale, publicly available query log from a Chinese commercial search engine, Sogou.com, namely . 
To evaluate the performance of our framework, we conduct experiments on a large-scale public available benchmark data (Tiangong-ST~\footnote{\url{http://www.thuir.cn/tiangong-st/}.}~\cite{chen2019sogou}) and a released testing set from Sogou-QCL~\footnote{\url{http://www.thuir.cn/sogouqcl/}.}~\cite{zheng2018sogou}.
Table~\ref{data_stat} shows the statistics of the datasets. 
Tiangong-ST provides web search session data from an 18-day search log. 
It contains weak relevance labels (i.e., click relevance labels~\cite{xiong2017end}) derived by six different click models for all query-document pairs and human relevance labels for documents in the last query of 2,000 sampled sessions. 
%We use the 2,000 last queries as our $Test_1$ set for an ad-hoc retrieval task.
To ensure efficiency when training the query reformulator, we exploit document titles in both training and testing instead of the full document content.
Similar experimental setups have been used in previous studies (e.g.,~\cite{lixs2018cikm}).
Prior studies~\cite{chuklin2015click, xiong2017end} have shown that weak relevance labels derived from click models can be used to train and evaluate retrieval models. 
Since the Partially Sequential Click Model (PSCM)~\cite{wang2015incorporating} achieves the best relevance estimation performance among the six click model alternatives, we employ click labels from the PSCM for training and validation. 
Training on weak relevance labels also enables our pipeline to obtain an immediate reward about the ranking results.

We evaluate our framework on two datasets: Tiangong-ST testing set and Sogou-QCL testing set. Tiangong-ST testing set is built from the last query of 2,000 sampled sessions. We use click relevance labels from the same PSCM and the provided five-graded human annotated relevance labels for evaluation. 
In Sogou-QCL testing set, we used click relevance labels from PSCM for evaluation. 


%Following the experimental setups in previous works~\cite{xiong2017end,liu2018entity}, we utilize three different relevance labels to evaluate our model on the test set.
%In the Test-SAME setting, we uses click relevance labels from the same PSCM and the provided five-graded human annotated relevance labels to evaluate our model. 


%In the Test-DIFF setting, we use the Dynamic Bayesian Network click model (DBM)~\cite{dupret2008user} as the relevance labels for evaluation. 

%In HUMAN-label setting, we use the provided five-graded human annotated relevance labels to evaluate ranking performance.

\textbf{Entity annotation}: We utilize XLore~\cite{xlore2013} as our knowledge graph foundation. XLore is an English-Chinese bilingual knowledge graph built from English Wikipedia, Chinese Wikipedia, Baidu Baike and Hudong Baike. It contains 16,284,901 entities, 2,466,956 concepts and 446,236 relations. The relations have four types: \textit{subclass}, \textit{instanceof} and \textit{same}, \textit{related}, where the proportions are 2.6\%, 42.1\%, 7.9\%, 47.3\%, respectively. 
The relations \textit{subclass} and \textit{instanceof} are further categorized as Derivation type while \textit{same} and \textit{related} are considered to be Equivalency type. 
These relations discover more relevant items compared with PRF and thus provide potential to improve query reformulation.
The distribution of the entity number in the query in the training set is shown in Figure~\ref{entity_number}, where over 95.9\% of queries have at least one entity and the average entity number in the query is 3.44.

%The query and document entities are annotated by CMNS~\cite{2017Entity}, the commonness (popularity) based entity linker, which follows the settings of previous work~\cite{liu2018entity}. 


\textbf{Candidate terms}: The candidate terms come from two sources: pseudo relevance feedback and knowledge information. We use the terms from top 3 documents retrieved by BM25 as the pseudo relevance feedback terms (17.2 terms on average). 
%For knowledge information, we study two strategies as discussed in Section~\ref{know_extrac_section}. 
Knowledge terms are first filtered if they are duplicated with PRF terms. 
Specifically, we keep the top 20 terms according to the embedding similarity with the query terms as the knowledge enhanced candidate terms. 
The number of expanded terms $K$ is set as 3~\footnote{We find expanding more than 3 terms do not have significant difference on retrieval performance but it increases much training time. Thus expanding 3 terms is a suitable setting in our work.}.
%Note that the number of terms from two sources is adjustable. 
%As discussed in~\cite{brandao2014learning}, a suitable term number is required to balance the retrieval efficiency and retrieval performance. 
%In our work, we 
%Therefore, we use 20 terms to enable fast training and effective retrieval performance. 
%In addition, we set the number of expanded terms $K$ as 3 and we will also discuss other settings in Section~\ref{para_analysis}.

\begin{figure}[!t]
	\centering
	%\setlength{\abovecaptionskip}{0pt}
	%\setlength{\belowcaptionskip}{10pt}
	%\vspace{-2mm}
	\includegraphics[scale=0.20]{fig/query_count}
	\caption{The distribution of entity number in the query.}
	\label{entity_number} %% label for entire figure
	%\vspace{-2mm}
	%avg: q: 3.4368355, d: 4.92020
\end{figure}



\subsection{Experimental Settings}
Since our pipeline consists of automatic query reformulation and neural retrieval model, we compare our pipeline with existing neural retrieval models and study the effectiveness of different query reformulation methods in our pipeline .
\subsubsection{Retrieval Model Baselines}
%To illustrate the effectiveness of our knowledge-aware automatic query reformulation framework, we compare our framework with the following baselines and details their parameter settings. Specifically, Model-PRF and Model-KNOW refer to the methods with PRF terms only and the combination of knowledge terms and PRF terms, respectively.

\begin{table*}[!t]
	\centering
	\caption{Retrieval performance of our CNIR pipeline with existing retrieval models. The subscript $P$ and $K$ denote the PRF and Knowledge enhanced candidate term set, respectively.
		$\dagger$, $1$ and $2$ indicate statistically significant improvements over the strongest baseline BERT, the
		original ranker in CNIR (i.e., KNRM or BERT) and the corresponding CNIR{$_p$}. (p-value $\leq$ 0.05)}
	\small
	\begin{tabular}{lcccc|cccc|cccc}
		\toprule
		& \multicolumn{4}{c|}{\textbf{PSCM} (Tiangong-ST)}                                & \multicolumn{4}{c|}{\textbf{HUMAN} (Tiangong-ST)}                                 & \multicolumn{4}{c}{\textbf{PSCM} (Sogou-QCL)}                               \\ \midrule
		& \textbf{MAP} & \textbf{ERR} & \textbf{ndcg@5} & \textbf{ndcg@10} & \textbf{MAP} & \textbf{ERR} & \textbf{ndcg@5} & \textbf{ndcg@10} & \textbf{MAP} & \textbf{ERR} & \textbf{ndcg@5} & \textbf{ndcg@10} \\ \midrule
		BM25                                            & 0.4577                                                               & 0.2928                                                               & 0.4474                                                               & 0.6207                                     & 0.7743                           & 0.4390                                                               & 0.6269                                                               & 0.7890                                                               & 0.6064                        & 0.4322                        & 0.4790                           & 0.5949                            \\
		ARCII &0.6803&0.3650&0.6866&0.7854&0.7819&0.4581&0.6889&0.8285&0.6035&0.4283&0.4821&0.6011\\
		ARCI &0.6929&0.3944&0.7012&0.7946&0.7854&0.4673&0.7043&0.8256&0.6023&0.4345&0.4904&0.6056\\
		DSSM &0.7112&0.4312&0.7143&0.8043&0.7842&0.4701&0.7016&0.8253&0.6056&0.4408&0.4989&0.6135\\ \hline
		KESM &0.7294&0.4793&0.7447&0.8459&0.7847&0.4789&0.6989&0.8345&0.6171&0.4526&0.5163&0.6293\\
		EDRM &0.7971&0.4912&0.8106&0.8645&0.7984&0.5032&0.7135&0.8389&0.6224&0.4752&0.5519 & 0.6422\\ \hline
		KNRM                                            & 0.7748                                                               & 0.4948                                                               & 0.7885                                                               & 0.8507                                     & 0.8051                           & 0.5002                                                               & 0.7119                                                               & 0.8374                                                               & 0.6044                        & 0.4485                        & 0.4960                           & 0.6099                            \\
		\textbf{CNIR$_{P}$ + KNRM}                                        & 0.7901\rlap{$^{1}$}                                                                           & 0.5020                                                               & 0.8098\rlap{$^{1}$}                                                               & 0.8621\rlap{$^{1}$}                                     & 0.8071                           & 0.5175\rlap{$^{1}$}                                                               & 0.7169                                                               & 0.8451                                                               & 0.6245\rlap{$^{1}$}                        & 0.4708\rlap{$^{1}$}                        & 0.5415\rlap{$^{1}$}                           & 0.6382\rlap{$^{1}$}                            \\
		\textbf{CNIR$_{K}$ + KNRM}             & {0.8135}\rlap{$^{1,2}$}                           & {0.5231}\rlap{$^{1,2,\dagger}$}                               & {0.8334}\rlap{$^{1,2}$}                             & {0.8845}\rlap{$^{1,2}$}      & {0.8097}                           & {0.5257}\rlap{$^{1}$}                                & {0.7212}                                                               & {0.8574}\rlap{$^{1}$}                                & {0.6398}\rlap{$^{1,2}$}                        & {0.4892}\rlap{$^{1,2}$}                        & {0.5741}\rlap{$^{1,2}$}                           & {0.6532}\rlap{$^{1,2}$}                            \\ \hline
		BERT                                            & 0.8273                                                               & 0.5012                                                               & 0.8422                                                               & 0.8822                                     & 0.8086                           & 0.5267                                                               & 0.7275                                                               & 0.8511                                                               & 0.6549                        & 0.5070                        & 0.5771                           & 0.6722                            \\
		\textbf{CNIR$_{P}$ + BERT}                                        & 0.8475\rlap{$^{1}$}                                                                & 0.5224\rlap{$^{1}$}                                                                & 0.8693\rlap{$^{1}$}                                                               & 0.9031\rlap{$^{1}$}                                      & 0.8093                           & 0.5277                                                               & 0.7285                                                               & 0.8519                                                               & 0.6727\rlap{$^{1}$}                         & 0.5277\rlap{$^{1}$}                         & 0.5886\rlap{$^{1}$}                            & 0.6947\rlap{$^{1}$}                             \\
		\textbf{CNIR$_{K}$ + BERT}            & \textbf{0.8735}\rlap{$^{1,2}$} & \textbf{0.5426}\rlap{$^{1,2}$} & \textbf{0.8864}\rlap{$^{1,2}$} & \textbf{0.9073}\rlap{$^{1}$}           & \textbf{0.8104} & \textbf{0.5383}\rlap{$^{1,2}$} & \textbf{0.7405}\rlap{$^{1,2}$} & \textbf{0.8649}\rlap{$^{1,2}$} & \textbf{0.6860}\rlap{$^{1,2}$}                        & \textbf{0.5367}\rlap{$^{1,2}$}                        & \textbf{0.5980}\rlap{$^{1,2}$}                           & \textbf{0.7063}\rlap{$^{1,2}$}                            \\ 
		\bottomrule                  
	\end{tabular}
	\label{nrm_baseline}
\end{table*}

\begin{itemize}[leftmargin=*,nosep]
	\item \textbf{BM25}: A popular probabilistic bag-of-words retrieval function that ranks a set of documents based on the query terms appearing in each document~\cite{robertson1994some}.
	\item \textbf{ARCII}~\cite{hu2014convolutional}: A neural retrieval model that maps the word embeddings of query and document to an aggregated embedding by a CNN. we use a two-layer CNN, where the size of kernels and pooling in both layers are set to (3 $\times$ 3) and (2 $\times$ 2). There are 16/32 kernels in two layers.
	\item \textbf{ARCI}~\cite{hu2014convolutional}: ARCI is a representation-based model which encodes text information by CNNs. We use a three-layer CNN where the filter windows sizes are 1 to 3 and there are 64 feature maps for each filter.
	\item \textbf{DSSM}~\cite{huang2013learning}: DSSM is also a representation-based model. It consists of a word hashing layer, two non-linear hidden layers, and an output layer. We use a three-layer DNN as in the original paper of DSSM; the hidden number of each layer is set to 50.
	\item \textbf{KESM}~\cite{xiong2018towards}: KESM is knowledge-aware neural retrieval model baseline, which models the salience of query entities in candidate documents. We set the dimension of word and entity embedding as 50 and remains other parameter settings as the original paper.	
	\item \textbf{EDRM}~\cite{liu2018entity}: EDRM is another knowledge-aware neural retrieval model, which considers both semantic similarity and entity relationship. We set the dimension of word and entity embedding as 50 and remains other parameter settings as the original paper.
	\item \textbf{KNRM}~\cite{xiong2017end} : 
	We use 11 kernels as the default setting in the original paper (10 soft-matching and 1 exact-matching kernels).
	\item \textbf{BERT}~\cite{devlin2018bert} : The state-of-the-art neural retrieval model. We use the pretrained 12-layer \textit{bert-base-chinese}\footnote{\url{https://github.com/google-research/bert/blob/master/multilingual.md}} model.
\end{itemize} 

\subsubsection{Automatic Query Reformulation Baselines}

\begin{itemize}[leftmargin=*,nosep]

	\item \textbf{TFIDF}: We extract the terms with top $K$ TFIDF values and add them to the original queries to test the retrieval performance.
	\item \textbf{RM}: RM is the Lavrenko's relevance models~\cite{croft2001relevance}, which is a popular relevance model for query reformulation. We follow the setting in~\cite{zhai2004study} and set the parameter $\lambda=0.5$. 
	\item \textbf{SL}: Following~\cite{cao2008selecting}, we implement a recurrent neural network (RNN) as the Supervised Learning baseline (SL). We feed query terms into RNN and take the last output embedding as the query representation. Then it is concatenated with the candidate terms to form the state representation, which is feed into a feed-forward neural network to estimate the probability of this word to be chosen. The term is marked as relevant if $(R' - R) > 0.3$, where $R'$ and $R$ are the retrieval performance of the reformulated query and the original query, respectively.
	\item \textbf{RL-CNN}~\cite{nogueira2017task}: The recent Reinforcement Learning (RL) query reformulation method. To fairly compare its performance, the CNN architecture is the same as our query reformulator. When it is applied on knowledge enhanced candidate terms, it is the same as our query reformulator in Section~\ref{reformulator_section}.%The retrieval model is BM25.
\end{itemize} 

\subsubsection{Parameter settings}
%We implement our models using Pytorch. 
The parameters of the query reformulator are optimized by Adagrad optimizer, with a batch size of 50 and a learning rate of 1e-5. Neural retrieval models are trained with Adam optimizer. The learning rate of KNRM during pretraining and fine-tuning is 1e-3 and 1e-4 while BERT always uses a learning rate of 3e-6. The dimension of the word embeddings, entity embedding are both 50. Word embeddings are pretrained on a Chinese Wikipedia dataset while entity embeddings are pretrained on the given graph structure by node2vec~\cite{Aditya2016}\footnote{We do not use the popular TransE~\cite{Antoine2013} to pretrain entity embedding because the number of relation types in XLore is small.}.  For the CNN layer in the query reformulator, the filter windows sizes are 1 to 3 and there are 50 feature maps for each filter. Early stopping with a patience of 10 epochs is adopted during the training process. For each query, we sample 5 possible reformulated queries, i.e., $M=5$.  For neural retrieval models, KNRM and BERT are updated after the query reformulator learns for 10 and 20 epochs, respectively. The source code is publicly available\footnote{\url{https://github.com/lixsh6/WSDM2022-CNIR}.}.


%Can it effectively improve the ranking performance of three different retrieval models?
\vspace{-1mm}
\section{Evaluation results}
In this section, we present our experimental results to answer the following research questions: \begin{enumerate}[leftmargin=*,nosep,label=(RQ\arabic*)]
	\item How does our pipeline perform compared to existing neural retrieval models?
	\item How does our pipeline perform when using other query reformulation methods?
	\item Does cooperative training strategy boost the ranking performance of our pipeline?
	\item How efficient is our pipeline in both training and testing?
\end{enumerate}
\vspace{-1mm}

\subsection{Overall ranking performance}
This section aims to answer $\bm{RQ1}$. 
We first compare our pipeline with different retrieval model baselines, which includes BM25, neural IR models and knowledge-aware neural IR models (KESM and EDRM).
The results are shown in Table~\ref{nrm_baseline}.

It is observed that our CNIR pipeline conducted on PRF and Knowledge candidate terms (CNIR$_{P}$ and CNIR$_{K}$) can outperform BM25, neural IR models and knowledge-aware neural IR models in most evaluation metrics.
This shows the retrieval power of our pipeline across different retrieval models.
For the comparison with the original neural retrieval model in CNIR pipeline, we find CNIR can significantly improves the ranking performance of KNRM and BERT in most evaluation metrics.
Though, the improvements over human annotated labels in Tiangong-ST are not all significant, it may be because that our pipeline CNIR is trained with pseudo relevance label PSCM, which is somehow inconsistent with human labels.
In general, it illustrates that our pipeline with additional automatic query reformulation can effectively improve the ranking performance of the original neural retrieval model.
Query reformulator, with the goal of optimizing the ranking metric of a given document list, can learn to generate a better query that represents users' information needs. 
Due to the improved query, the neural retrieval model can also estimate the relevance of each document better and improve the ranking performance again.
Two modules learn from each other and continuously optimize the ranking performance during training.

We also compare our pipeline when incorporating knowledge information into automatic query reformulation.
Note CNIR$_{K}$ is not only different with CNIR$_{P}$ from the perspective of candidate term construction, but also the additional entity inputs to the CNN architecture in Equation~\ref{input_eq}.
It is observed that when using knowledge information CNIR$_{K}$ can outperform CNIR$_{P}$ significantly in most evaluation metrics on KNRM and BERT.
On human annotated labels in Tiangong-ST, CNIR$_{K}$ is also superior to the original BERT significantly on ERR, ndcg@5,10. 
It suggests that the performance of automatic query reformulation decides the upper bound of ranking performance in our pipeline.
If automatic query reformulation is improved, the ranking performance of the pipeline can be better during the cooperative learning process.
 

\begin{table}[t]
	\centering
	\caption{Comparison with other automatic query reformulation methods in CNIR$_{K}$.  
		$\dagger$ indicate significant improvements over the original ranker (Raw). (p-value $\leq$ 0.05)}
	\small
	
	\begin{tabular}{p{1.8cm}cc|cc}
		\toprule
		& \multicolumn{2}{c|}{ Tiangong-ST}                                                             & \multicolumn{2}{c}{ Sogou-QCL}                                                             \\ \midrule
		& \textbf{ ndcg@5}                     &  \textbf{ ndcg@10}                                & \textbf{ ndcg@5}  & \textbf{ ndcg@10} \\ \midrule
		%Raw-BM25  & 	0.4474& 0.6207 	& 0.6269& 	0.7890                      \\ \midrule
		\specialrule{-0.1pt}{0pt}{0.pt}\multicolumn{4}{l}{\fontsize{8}{10} \textbf{BM25 as ranker}}  \\ \midrule
		Raw 	&0.4474&0.6207&0.4790&0.5949\\                
		TFIDF                      & 0.4435                     & 0.6318                                         & 0.4112                     & 0.5305                      \\
		RM                        & 0.4174                     & 0.6165                                        & 0.3892                     & 0.4978                      \\
		SL                         & 0.4694\rlap{$^{\dagger}$}  &	0.6384\rlap{$^{\dagger}$}  & 0.5053\rlap{$^{\dagger}$}  &	0.6271\rlap{$^{\dagger}$} \\ 
		RL-CNN                         & {0.4815}\rlap{$^{\dagger}$}  & 0.6275   & 
		{0.5124}\rlap{$^{\dagger}$} & 0.6242\rlap{$^{\dagger}$}\\ 
		\midrule
		\specialrule{-0.1pt}{0pt}{0.pt}\multicolumn{4}{l}{\fontsize{8}{10} \textbf{KNRM as ranker}}  \\ \midrule  
		Raw 	&0.7885&0.8507&0.4960&0.6099\\   
		TFIDF                      & 0.7313                    & 0.7905                                        & 0.4760                    & 0.5829                      \\
		RM                        & 0.7283                     & 0.7823                                       & 0.4693                     & 0.5702                      \\
		SL                         & 0.8105\rlap{$^{\dagger}$} &	0.8671\rlap{$^{\dagger}$} & 0.5312\rlap{$^{\dagger}$} &	0.6254\rlap{$^{\dagger}$}\\ 
		CNIR(RL-CNN)   & {0.8334}\rlap{$^{\dagger}$}  & 0.8845\rlap{$^{\dagger}$}    & 
		{0.5741}\rlap{$^{\dagger}$}  & 0.6532\rlap{$^{\dagger}$}   \\
		 \hline
		\specialrule{-0.1pt}{0pt}{0.pt}\multicolumn{4}{l}{\fontsize{8}{10} \textbf{BERT as ranker}}  \\ \midrule  
		Raw 	&0.8422&0.8822&0.5771&0.6722\\   
		TFIDF                      & 0.8252                     & 0.8626                                         & 0.5471                     & 0.6322                      \\
		RM                        & 0.8193                     & 0.8593                                        & 0.5413                    & 0.6315                      \\
		SL                         & 0.8538\rlap{$^{\dagger}$} &	0.8823 & 0.5874\rlap{$^{\dagger}$} &	0.6863\rlap{$^{\dagger}$}\\ 
		CNIR(RL-CNN)   & \textbf{0.8864}\rlap{$^{\dagger}$}  & \textbf{0.9073}\rlap{$^{\dagger}$}    & 
		\textbf{0.5980}\rlap{$^{\dagger}$}  & \textbf{0.7063}\rlap{$^{\dagger}$}   \\
		\bottomrule
	\end{tabular}
	\label{qr_baseline}
\end{table}


\begin{table}[t]
	\centering
	\caption{Ranking performance when freezing the parameters of neural retrieval model.}
	\small
	
	\begin{tabular}{p{1.8cm}cc|cc}%{p{2.5cm}p{1.05cm}p{1.05cm}|p{1.05cm}p{1.05cm}}
		\toprule
		& \multicolumn{2}{c|}{ Tiangong-ST}                                                             & \multicolumn{2}{c}{ Sogou-QCL}                                                             \\ \midrule
		& \textbf{ ndcg@5}                     &  \textbf{ ndcg@10}                                & \textbf{ ndcg@5}  & \textbf{ ndcg@10} \\ \midrule
		%Raw-BM25  &  0.4474& 0.6207  & 0.6269&  0.7890                      \\ \midrule
		\specialrule{-0pt}{0pt}{0.pt}\multicolumn{4}{l}{\fontsize{8}{10} \textbf{KNRM as ranker}}  \\ \hline
		CNIR$_{P}$ (Freeze)  & 0.7764                            & 0.8412                             & 0.5342                            & 0.6289                             \\
		CNIR$_{P}$            & 0.8089                            & 0.8621                             & 0.5415                            & 0.6382                             \\
		CNIR$_{K}$ (Freeze) & 0.8123                            & 0.8615                             & 0.5351                            & 0.6270                             \\
		CNIR$_{K}$          & 0.8334                            & 0.8845                             & 0.5741                            & 0.6532                             \\ \hline
		\specialrule{-0.1pt}{0pt}{0.pt}\multicolumn{4}{l}{\fontsize{8}{10} \textbf{BERT as ranker}}  \\ \hline
		CNIR$_{P}$ (Freeze)  & 0.8451                            & 0.8844                             & 0.5711                            & 0.6873                             \\
		CNIR$_{P}$           & 0.8693                            & 0.9031                             & 0.5886                            & 0.6947                             \\
		CNIR$_{K}$ (Freeze) & 0.8421                            & 0.8852                             & 0.5732                            & 0.6892                             \\
		CNIR$_{K}$          & \textbf{0.8864}                            & \textbf{0.9073}                             & \textbf{0.5980}                            & \textbf{0.7063}    \\
		\bottomrule
	\end{tabular}
	\label{train_alternate}
\end{table}

\subsection{Analysis on query reformulation}
This section aims to answer $\bm{RQ2}$. 
We alter the RL based automatic query reformulation method in our pipeline to compare the effectiveness of other query reformulation methods.
In addition to neural retrieval models, we also include BM25 as the retrieval model in our pipeline. The results are shown in Table~\ref{qr_baseline}.
In the scenario with BM25 ranker, our pipeline deteriorates the traditional query reformulation optimization~\cite{cao2008selecting,nogueira2017task} where retrieval models do not require to be trained.
$Raw$ indicates that the original retrieval model without automatic query reformulation.
In the scenario with neural retrieval models, we compare the rule-based query reformulation strategy $TFIDF$, $RM$ and a supervised learning method $SL$.
Note our query reformulator has the same structure with RL-CNN, RL-CNN with KNRM or BERT indicates our CNIR pipeline.

We find it is hard to improve the ranking performance when applying our pipeline on BM25, rule-based methods cannot improve the ranking performance of BM25. 
It suggests that both rule-based methods cannot capture the effective terms in relationship with the original query.
Supervised learning and reinforcement learning methods learn to reformulate queries according to the feedback of ranking performance, thus are effective to improve the ranking performance of the original ranker BM25.
Since RL-CNN learns with a continuous reward against the discrete signal in SL, RL-CNN can distinguish the useful terms better for query reformulation and thus achieves better ranking performance. 


When applying neural retrieval models in our pipeline, we find the ranking performance is consistent to the quality of automatic query reformulation methods. Rule-based query reformulation is not effective in our pipeline while supervised learning and reinforcement learning methods contribute to better ranking performance. This phenomenon suggests that the quality of automatic query reformulation methods decides how well the whole pipeline can achieve. This also motivates us to build a knowledge enhanced query reformulator to further improve the ranking performance.

\vspace{-1mm}
\subsection{Analysis on cooperative training}
This section aims to answer $\bm{RQ3}$. 
We aim to understand how our pipeline performs when it deteriorates to the traditional automatic query reformulation optimization (i.e., the retrieval models are not required to be trained.)
We freeze the parameters of neural retrieval models and only train the query reformulator to validate the necessity of our proposed cooperative training strategy. 
The results are shown in~Table~\ref{train_alternate}.

It is found that regardless of candidate terms construction, if KNRM and BERT are not fine-tuned during the training, they cannot perform well on the reformulated queries.
It is because neural retrieval models are not trained with these reformulated queries. 
The relevance estimation of these queries may not be accurate and thus yields a wrong signal to train query reformulator.
In this scenario, the learning of query reformulator is limited by the ranking power of current neural retrieval models.
Ideally, when the power of the query reformulator achieves a upper bound after certain epochs, it captures the possible reformulated queries that the current retrieval models can do well.
Thus, it is necessary to conduct cooperative training strategy to make sure both query reformulator and neural retrieval models can be optimized continuously.


\vspace{-1mm}
\subsection{Time efficiency}
This section aims to answer $\bm{RQ4}$. 
Since our pipeline exploits additional automatic query reformulation module compared to other retrieval models, we aim to understand whether it increases acceptable time overheads.
We report the time consumption of different retrieval frameworks, as shown in Table~\ref{time}. 
Automatic query reformulation is based on knowledge enhanced candidate terms.


The parameter number of our query reformulator is about 5 million. 
Neural retrieval model is the key module in our pipeline while the parameters in query reformulator is far less than those in the neural retrieval models.
Therefore, neural retrieval models with larger complexity require more training time in our pipeline.
We can observe that the query reformulator only increases negligible time on the original rankers during inference. 
However, our pipeline brings significant improvements to the original neural retrieval models.
As reported in Table~\ref{nrm_baseline}, CNIR$_K$ + KNRM can perform closely to BERT while its efficiency is substantially superior to BERT. 
This makes our framework computationally applicable in practical ranking systems.


\begin{table}[!t]
	\centering
	\caption{Comparison of time consumption over Tiangong-ST testing set when using different retrieval frameworks. }
	\small
	\begin{tabular}{lccc}
		\toprule
		& \textbf{\#params} & \textbf{\begin{tabular}[c]{@{}c@{}}Training\\ (total time)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Testing\\ (full test set)\end{tabular}} \\ \midrule
		BM25 & n.a                & n.a                                                                     & 1.2s \\
		RL-CNN & 5M                & 3.2h                                                                     & 1.3s                                                                       \\ \midrule
		KNRM & 5M & n.a & 1.3s\\
		CNIR$_K$ + KNRM & 10M               & 9.4h                                                                     & 1.4s                                                                       \\ \midrule
		BERT & 103M & n.a & 49.5s\\
		CNIR$_K$ + BERT & 108M              & 38.3h                                                                    & 52.2s      \\
		\bottomrule                                                               
	\end{tabular}
	\label{time}
\end{table}










==> sections/introduction.tex <==
% !TEX root =  ../wsdm2022-fp-xiangsheng.tex

\section{Introduction}
\label{introduction}
%Compared with traditional IR models like BM25 and \textit{learning to rank} (L2R) methods~\cite{lucchese-2019-learning}, neural retrieval models learn semantic representation directly from the raw text rather than hand-crafted IR features and achieve significantly better ranking performance in a wide range of ranking applications~\cite{xiong2017end,qiao2019understanding}.

Neural retrieval models learn distributed representations of query and documents and conduct semantic matching in the embedding space~\cite{xiong2017end}.
A bottleneck of information retrieval is that the short queries issued by users may vaguely represent their true information needs~\cite{mitra2017neural}.
According to the investigations conducted on large-scale commercial search engines, a query often contains less than three terms and over 16\% of queries are ambiguous~\cite{li2018hierarchical}. 
Therefore, to accurately understand users' search intents behind these queries is challenging for search engines.
To a certain extent, these queries limit the upper bound of ranking performance in existing neural retrieval models.

To address this problem, automatic query reformulation technique~\cite{nogueira2017task} is proposed to alter a given query to better represent user's search intent and improve retrieval performance. 
The basic idea of these methods is to extract terms from top retrieved documents (which is called pseudo-relevance feedback (PRF)) and select terms to expand the original query.
Automatic query reformulation has been demonstrated effective and necessary in information retrieval in many applications~\cite{croft2001relevance,xu2017quary,nogueira2017task}. 
However, these studies consider query reformation as an independent learning task before ranking task and do not consider its interactions with the following ranking models.
This motivates us to build an integral framework with query reformulation and ranking models.


In this paper, we design a new Cooperative Neural Information Retrieval pipeline (CNIR) with automatic query reformulation. The framework is shown in Figure~\ref{pipeline}.
Different from the traditional neural IR framework, we incorporate a parameterized query reformulation module before neural retrieval model.
User-issued query is first reformulated with an automatic query reformulator and then passed to the following neural retrieval model. 
%The goal of the proposed pipeline is similar to traditional neural IR framework, which is to offer the best ranking results to the user.
Inside the pipeline, automatic query reformulator and neural retrieval models aim to optimizing the quality of reformulated queries and ranking performance, respectively. 
Two modules learn from the feedback of each other to improve the ranking performance, where query reformulator provides the queries with better quality to neural retrieval models while the neural retrieval model returns the ranking results and the corresponding ranking metric to query reformulator.


The automatic query reformulator is based on reinforcement learning.
The \textit{action} is to sample $K$ terms to expand the original query while the \textit{reward} is the ranking performance metrics of the ranked lists retrieved by the original query.
Therefore, the query reformulator can generate better queries by learning to maximize the reward through training. 
For neural retrieval model, it takes as input the reformulated query instead of the original query. 
The reformulated query with better quality is assumed to better represent users' information needs and thus to achieve a better ranking performance than the original query.
We exploit an alternate training strategy to jointly optimize the query reformulator and the neural retrieval model in our pipeline, i,e., the parameters of one module is fixed while training the other.
Two modules are prompted alternately to reformulate better queries and improve retrieval performance.





%are categorized into two classes: query expansion~\cite{nogueira2017task} and query rewriting~\cite{bibid}. Query expansion typically expand the original query by adding potential relevant terms to form a query with clearer intent description while query rewriting targets to rewrite the original query to several alternative queries that can improve retrieval performance. The candidate

%dictionaries of synonyms~\cite{miller1995wordnet}

%Previous works on automatic query reformulation primarily expand the original query using pseudo-relevance feedback (PRF)~\cite{xu2017quary}. 
%PRF is shown effective in providing relevance signals in question-answering~\cite{yang2018response} and web search~\cite{zamani2016pseudo}.
%The basic idea of these methods is to extract terms from top retrieved documents to expand the original query, because these documents are assumed to be relevant to the query.
%However, this assumption is often invalid when the original query is misinterpreted by the search systems and the retrieved documents are not relevant to the query.
%To address this problem, more sophisticated mechanisms for selecting effective feedback documents~\cite{he2009finding} and effective expansion terms~\cite{cao2008selecting} are prompted.

To further improve the quality of the reformulated query, we incorporate knowledge information into the automatic query reformulation.
Previous works on automatic query reformulation primarily expand the query using pseudo-relevance feedback (PRF) (e.g., top retrieved documents)~\cite{xu2017quary}. 
However, PRF is often invalid when the original query is misinterpreted by the search systems and the top retrieved documents are not relevant to the query.
In general, knowledge offers two types of information: the relationships between entities, which are often represented as a (knowledge) graph, and the descriptions of entities.
Both types of knowledge are useful for automatic query reformulation. 
For example, in Figure~\ref{demo}, a user issues a query ``Bert character'' to find a muppet character. 
Retrieved documents from PRF are mostly about the pretrained language model, which do not match the user's search intent.
Knowledge information provides accurate information about the television show and thus can be used to reformulate a better query.

\begin{figure}[!t]
	\centering
	 \includegraphics[scale=0.25]{fig/example}
	%\includegraphics[clip,trim=0mm 0mm 0mm 2mm,width=\columnwidth]{fig/example}
	\caption{An example of using knowledge information for query reformulation.}
	\vspace{-2mm}
	\label{demo}
\end{figure}


 

%In this paper, we construct a knowledge-aware automatic query reformulation framework that leverages external knowledge information and learns to reformulate queries with reinforcement learning.
%The candidate terms for query reformulation are selected not only from the PRF terms but also the external knowledge information related to the entities in the original query.
%As shown by the example in Figure~\ref{demo}, when the PRF terms are not relevant to user's search intent, knowledge graphs can provide some additional terms which may make the candidate set more comprehensive, and therefore, more likely to cover user's intent. 
%Our framework uses a reinforcement-learning based reformulator agent to reformulate queries.
%The \textit{action} of the reformulator agent is to select or to drop a candidate term.
%As the goal is to optimize the ranking performance of the reformulated queries, we define the \textit{reward} as the ranking performance metrics of the ranked lists retrieved by the reformulated queries. Therefore, the reformulator agent would learn to generate better queries by learning to maximize the reward through training. 
%
%While we can apply our framework with different retrieval models (e.g., probabilistic relevance models and neural retrieval models), we find that when using a neural retrieval model, we can also fine-tune the retrieval model with the newly reformulated queries and improve its ranking performance by a substantial margin.
%Therefore, we further propose an alternate training strategy to jointly optimize the reformulator agent and the neural retrieval model.
%%The goal is to simultaneously optimize the quality of reformulated queries as well as the retrieval performance of neural retrieval models.
%When we train the reformulator agent to reformulate a better query, the parameters of the rankers are fixed.
%%The reformulator agent takes the neural retrieval models as the ranking environment while neural retrieval models are fine-tuned by the newly reformulated queries from the reformulator agent.
%After a certain epochs, the parameters of the reformulator agent are fixed and the rankers are fine-tuned based on the reformulated queries generated by the reformulator agent.
%Two components are prompted alternately to reformulate better queries and improve retrieval performance, the parameters of one is fixed while training the other.
%Two components are prompted alternately to reformulate better queries and improve retrieval performance.




To verify the flexibility and effectiveness of the proposed framework, we test the proposed pipeline with two neural retrieval models in this study, including a kernel based neural ranking model, KNRM~\cite{xiong2017end} and a pretrained contextualized ranking model (BERT)~\cite{devlin2018bert}. 
We conduct experiments on a large-scale public test collection~\cite{chen2019sogou} Tiangong-ST and a released testing set from Sogou-QCL~\cite{zheng2018sogou}. 
Experimental results show that our pipeline can effectively improve the retrieval performance of neural retrieval models. 
Meanwhile, we find using knowledge information to build automatic query reformulation module can further improve the ranking performance of our pipeline. 
Finally, we show that the time overheads introduced by our framework is acceptable for practical retrieval systems.

{The primary contributions of our work are three-folds}:
%	\item We develop a reinforcement learning framework that utilizes both pseudo relevance feedback and knowledge information for automatic query reformulation. 
%\item The proposed  framework is able to be applied to any retrieval models. In this study, we test the proposed framework with three representative retrieval models (BM25, KNRM and BERT). For neural retrieval models, we propose to alternatively train the rankers and reformulator agent, which further boosts the retrieval performance.
\begin{enumerate}[leftmargin=*,nosep]
	\item We present a Cooperative Neural Information Retrieval pipeline (CNIR) with automatic query reformulation, where query reformulation and neural retrieval model in the pipeline are optimized alternately from the feedback of each other.
	\item We incorporate knowledge information to build a knowledge enhanced query reformulation module, which further improve the ranking performance of the proposed pipeline. 
	\item Extensive experiments on two public test collections show that our pipeline effectively improves the retrieval performance of two representative neural retrieval models and the pipeline is also computationally acceptable for practical retrieval systems. 
	%We systematically analyze the effectiveness of external knowledge in different ranking scenarios, thereby providing a solid understanding of how to utilize external knowledge for automatic query reformulation.
\end{enumerate}



==> sections/method.tex <==
% !TEX root =  ../wsdm2022-fp-xiangsheng.tex

%\vspace{-1mm}
\section{Pipeline Framework}
%Cooperative Neural Information Retrieval
\label{method}
%This section presents our proposed knowledge-aware query reformulation framework. 
%The workflow of the overall framework is shown in Figure~\ref{workflow}. Below, we describe their details. 

%\begin{figure}[!t]
%	\centering
%	%\setlength{\abovecaptionskip}{0pt}
%	%\setlength{\belowcaptionskip}{10pt}
%	%\vspace{-2mm}
%	\includegraphics[scale=0.38]{fig/workflow2}
%	\caption{Knowledge-aware automatic query reformulation framework.}
%	%
%	\label{workflow} %% label for entire figure
%	%\vspace{-2mm}
%\end{figure}

\subsection{Overview}
\label{overview}
\begin{figure*}
	\centering
	\includegraphics[width=0.58\linewidth]{fig/pipeline}
	\caption{The framework of the proposed Cooperative Neural Information Retrieval pipeline (CNIR). Query reformulator is exploited in both training and inference stage in CNIR pipeline.}
	\label{pipeline}
\end{figure*}

The overall framework of our proposed Cooperative Neural Information Retrieval (CNIR) pipeline is shown in Figure~\ref{pipeline}. 
The pipeline is based on the assumption that queries with better quality can better represent users' information needs and thus achieve a better ranking performance than the original query~\cite{dai2019deeper}.
Compared with the traditional neural IR pipeline, our pipeline first reformulates the original query by a query reformulator and then takes the reformulated query as inputs into neural retrieval model.
The ranking results of the reformulated queries are passed back to the query reformulator and yield ranking metrics as a feedback signal to reflect the quality of the reformulated query.
For the neural retrieval model, it uses the reformulated query instead of the original query as inputs to optimize the ranking performance.
Two modules in the pipeline are alternately optimized with the feedback of each other.
Details of two modules are described as follows.

\subsection{Automatic Query Reformulation}
Automatic query reformulation module is based on reinforcement learning (RL), which can be divided into two parts: 1) candidate terms construction; 2) automatic query reformulation with RL.

\subsubsection{Candidate terms construction} 
\label{know_extrac_section}
Besides the top retrieved documents (i.e., PRF), candidate terms for automatic query reformulation are also from an external knowledge repository. 
We construct an entity linker to find knowledge information contained in the issued query.
To ensure efficiency, we apply an off-the-shelf entity linker to extract the entities in the query, namely the commonness (popularity) based entity linker~\cite{2017Entity}.
This linker identifies the query entities that are contained in a given large-scale knowledge repository.
According to the statistics of our experimental dataset in Figure~\ref{entity_number}, over 95.9\% of queries contain at least one entity in our dataset.
We then retrieve the neighbor entities that are connected to the query entities in the knowledge graph. The neighborhoods reveal the entities in the relationship of equivalency and derivation with the query entities, e.g., \textit{the United States}-\textit{USA} and \textit{Los Angles}-\textit{USA}, respectively. 

%knowledge information that is related to the query entities in the query by two strategies:

%\begin{enumerate}[leftmargin=*]%nosep
%	\item \textbf{Neighborhoods}: This method extracts the neighborhoods of the query entities as the knowledge information. The neighborhoods reveal the entities in the relationship of equivalency and derivation with the query entities, e.g., \textit{the United States}-\textit{USA} and \textit{Los Angles}-\textit{USA}, respectively. The details of our knowledge graph are described in Section~\ref{data_section}.	
%	\item \textbf{Descriptions}: This method exploits the entity descriptions as the knowledge information. Each description is about 100 words long. We merge the descriptions of all query entities as knowledge-based candidate terms.
%\end{enumerate}

To remove the noisy candidate terms, we further filter out the noisy terms according to their word embedding similarity with the query terms.
The top knowledge based candidate terms $\mathcal{C}_{know}$ with highest similarities are kept to combine with PRF terms $\mathcal{C}_{PRF}$ as the final knowledge enhanced candidate terms for the original query $q$, i.e., $\mathcal{C}_{q} = \mathcal{C}_{know} \cup \mathcal{C}_{PRF}$.
If there is no entity found in the query, the candidate terms only consist of the PRF terms as the previous work~\cite{nogueira2017task}, i.e., $\mathcal{C}_{q} = \mathcal{C}_{PRF}$.

\subsubsection{Automatic query reformulation with RL} 
\label{reformulator_section}
Given the knowledge enhanced candidate set $\mathcal{C}_{q}$, we aim to strategically select useful terms for automatic query reformulation.
The expanded query is required to boost the retrieval performance compared to the original query.
We thus exploit a reinforcement learning strategy to reformulate queries such that the retrieval performance under the reformulated queries is improved.
The architecture of our automatic query reformulator is shown in Figure~\ref{agent}.
%The reformulator takes an action of sampling $K$ candidate terms from $\mathcal{C}_{q}$ and expands the original query.
We then describe the \textit{State}, \textit{Action}, \textit{Reward}, and the learning via \textit{Policy Gradient}.


\textbf{State representation}:
The state represents whether a candidate term is suitable for the given query. 
Specifically, for a given query $\bm{q} = [w_1, w_2, \dots, w_n]$, we extract the entities that are contained in this query, denoting as $[e_1, e_2, \dots, e_m]$. 
The input sequence to the reformulator agent is denoted as the concatenation of the word and entity embedding $\bm{q}'=\{w_1, w_2, \dots, w_n, e_1, e_2, \dots, e_m \}$.
The convolutional layer of the agent is defined as:
\begin{equation}
	\label{input_eq}
	conv_i(z, \mathcal{K}_i) = MaxPool(ReLu(\phi(z)))
\end{equation}
where $z$ is the input features, $\phi$ is the convolutional operation; \textit{MaxPool} is the max-pooling operation and $\mathcal{K}_i$ is the kernels to be learned in the $i$th convolutional layer.

The query representation is then computed by multi-layer convolutional neural network, as follows:
\begin{equation}
	\begin{split}
		z_l & = conv_i(z_{l-1}, \mathcal{K}_l), l = 1,\dots,N
	\end{split}
\end{equation}
where $z_0 = \bm{q}' $ and the final query representation is $\hat{q}  = z_N$.

For each candidate term, we employ multi-layer neural networks to obtain a new vector representation $c'_j=MLP(c_j)$. 
The state representation is thus the concatenation between query representation and candidate vector representation:
\begin{equation}
	s_j = [\bm{q}' \circ c'_j]
\end{equation}

\textbf{Action}: 
The action is to sample $K$ candidate terms based on their state representation and append the sampled terms to the original query to form a new query.
The candidate terms are from the combination of PRF terms and knowledge based candidate terms in Section~\ref{know_extrac_section}, i.e., $\mathcal{C}_{q}$.
The action probability $\pi(s_j)  = P(c_j|\bm{q})$ of each candidate term is then estimated by:
\begin{equation}
	\label{sample_prob}
	\begin{split}
		P(c_j|\bm{q}) & = softmax(U^T tanh(W[\bm{q}' \circ c'_j]) + b)
	\end{split}
\end{equation}
where $U,W$ are the weights and $b$ is the bias. $K$ is the hyper-parameter in our experiment. Note each term is independently sampled by Equation~\ref{sample_prob} and the reward is obtained by inputting the newly reformulated query to the retrieval model.


\textbf{Reward}:
The goal of the query reformulator is to improve the ranking performance of the retrieved documents from the original queries, thus reward function can be any retrieval metrics. In our work, we use mean average precision (MAP) as the reward function. 

\textbf{Policy gradient}:
We train the query reformulator by REINFORCE algorithm~\cite{williams1992simple}. The gradient of the policy is given by 
\vspace{-4mm}

\begin{equation}
	\label{RL_target}
	\begin{split}
		\nabla & \mathcal{J}_{\Theta}(\Theta) = \mathbb{E}_{\pi_{\Theta}}\begin{bmatrix}\sum\limits_{k=1}^{K}{\nabla \log \pi (a_k|\Theta) } \cdot R  \end{bmatrix} \\
		& \approx \frac{1}{M}\sum\limits_{m=1}^{M}\sum\limits_{i=1}^{K}{\nabla \log \pi (a_k|\Theta)} \cdot R_m
	\end{split}
\end{equation}
\vspace{-3mm}

where $\Theta$ denotes the parameters of the query reformulator and $K$ is the number of expanded terms. $M$ is the sampled number. The expectation reward guides the updates of the parameters $\Theta$ of the agent policy $\pi(s_j)$. 

\begin{figure}[t]
	\centering
	%\setlength{\abovecaptionskip}{0pt}
	%\setlength{\belowcaptionskip}{10pt}
	%\vspace{-2mm}
	\includegraphics[scale=0.30]{fig/agent}
	\caption{Architecture of the automatic query reformulator.}
	%
	\label{agent} %% label for entire figure
	%\vspace{-3mm}
\end{figure}
\vspace{-1mm}
\subsection{Neural Retrieval Model Training}
\label{retrieval_model_section}
We take an assumption to train neural retrieval model in our pipeline: 
queries with better quality can better represent users' information needs and thus achieve a better ranking performance than the original query~\cite{dai2019deeper}.
Different from the previous work~\cite{voskarides2020query}, the retrieval model only processes the reformulated query.
It outputs the ranking results based on the retrieved documents from the original query.
In our work, we study two representative neural retrieval models, i.e., a kernel based neural ranking model (KNRM)~\cite{xiong2017end} and a pretrained contextualized ranking model (BERT)~\cite{devlin2018bert}.

\subsubsection{Kernel based Neural Ranking Model (KNRM)}
KNRM~\cite{xiong2017end} is a neural retrieval model that uses kernel pooling to model multi-level semantic similarity signals. Given word embeddings of a query and a document, it first constructs an interaction matrix $M$ to model word-level similarities, where each element in $M$ is the cosine similarity between a query word $w_i$ and a document word $w_j$:
\vspace{-1mm}
\begin{equation}
	M_{ij} = cos(\bm{v}_{w_i}^q, \bm{v}_{w_j}^d)
\end{equation}

where $\bm{v}_w$ is the word embedding of $w$. 
\textit{Kernel pooling} technique is then applied to map the interaction matrix into soft-matched ranking features. In particular, KNRM uses $T$ Gaussian kernels to count the soft matches of interaction pairs at $T$ different strength levels. Each kernel summarizes the interaction features in matrix $M$ as soft similarity counts in the region defined by its mean $\mu_t$ and width $\sigma_t$, generating a $T$-dimensional feature vector $\phi(M)=\{K_1(M), \dots, K_T(M)\}$:

\vspace{-3mm}
\begin{equation}
	\begin{split}
		K_t(M) & = \sum_i\log K_t(M_i) \\
		K_t(M_i) & = \sum_j \exp (-\frac{(M_{ij} - \mu_k)^2}{2\sigma_t^2})
	\end{split}
\end{equation}
%Prior studies have shown that such counting-based pooling methods can achieve better performance than score-based methods like mean-pooling or max-pooling~\cite{pang2017deep}. 
The final  relevance score is computed with a standard ranking layer:
\begin{equation}
	f(\bm{q},\bm{d}) = tanh(w_r \cdot \phi(M) + b_r) 
\end{equation}

with parameters $w_r$ and $b_r$ and $tanh$ activation layer. Compared with BM25, KNRM captures semantic relevance signals and obtains better retrieval performance~\cite{lixs2020cikm}.

\subsubsection{BERT} 
BERT~\cite{devlin2018bert} is a pretrained contextualized transformer based language model, which has shown state-of-the-art retrieval performance in many IR-related tasks~\cite{qiao2019understanding}. BERT concatenates the query and document into a text sequence and feeds it into a multi-layer pretrained transformer architecture:
%\vspace{-1mm}
\begin{equation}
	BERT(\bm{q},\bm{d}) = Transformers([CLS] \circ \bm{q} \circ [SEP] \circ \bm{d} \circ [SEP])
\end{equation}

The special token representation $[CLS]$ in the last layer is considered as the matching feature between query $\bm{q}$ and document $\bm{d}$. The ranking layer is applied to the matching feature to estimate the final relevance score:
\begin{equation}
	f(\bm{q},\bm{d}) = tanh(w_r \cdot BERT_{CLS}(\bm{q},\bm{d})+ b_r) 
\end{equation}

where $w_r$ and $b_r$ are the learning-to-rank parameters.  


\begin{algorithm2e}[t]
	\KwInput{Training collection $\mathcal{S} = \{(q_1, \bm{D}_1), \dots, (q_T, \bm{D}_T) \}$, where $\bm{D}_i=\{d_1, \dots, d_L\}$ is the document list of $q_i$, query reformulator (QR) and neural retrieval model (NRM).}
	\KwOutput{The ranking results of each $\bm{D}_i$.}
	%\KwData{Testing set $x$}
	%$\sum_{i=1}^{\infty} := 0$ \tcp*{this is a comment}
	%\tcc{Continue reading while stop reading signal is not positive}
	%\tcp*{Stop reading signal is not positive}
	\textbf{Pretrain} NRM with the training collection by Equation~\ref{rank_loss}.\\
	%\textbf{Initalize} variable $\textit{epoch}$ = 0;\\
	\While{convergence condition is not attained}{
		Freeze the parameters of NRM and unfreeze QR.\\
		\For{each sample $(q_i, \bm{D}_i)$ in $\mathcal{S}$}
		{
			QR reformulates $q_i$ to $q_i^{'}$ by Equation~\ref{sample_prob}.\\
			Compute the ranking metric $R_i$ based on the ranking results of $q_i^{'}$.\\
			Train QR by Equation~\ref{RL_target}.
		}
		\If{$\textit{epoch}$ \% TRAIN\_RANKER\_FRE == 0}
		{
			Freeze the parameters of QR and unfreeze NRM.\\
			\For{each sample $(q_i, \bm{D}_i)$ in $\mathcal{S}$}
			{
				QR reformulates $q_i$ to $q_i^{'}$ by Equation~\ref{sample_prob}.\\
				Train NRM with the sample $(q_i^{'}, \bm{D}_i)$ by Equation~\ref{rank_loss}.\\
			}
		}
		$\textit{epoch}$ = $\textit{epoch}$ + 1.\\
	}		
	\caption{Cooperative training of the CNIR pipeline.}
	\label{algo}
\end{algorithm2e}

\subsection{Cooperative Training Procedure}
\label{training_section}
Note that we do not retrieve documents again by the reformulated queries.
Instead, we aim to optimize the ranking performance of the retrieved documents from the original queries.
Automatic query reformulation module and neural retrieval model are learned based on the feedback of each other.
We propose an alternate training strategy to train our pipeline, as detailed in Algorithm~\ref{algo}.
We initialize the neural retrieval model by training on the original training collection.
For the training process of CNIR, the query reformulator is trained first with the reward obtained from the neural retrieval model. 
It encourages the reformulator to reformulate queries with better quality.
Then, the reformulated queries are used to fine-tune of the neural retrieval model, which facilitates the retrieval model to better estimate the document relevance.

%The idea is similar to contrastive learning with weak supervision data~\cite{sun2020meta}, where the neural retrieval model is improved with a larger dataset.


Two modules in CNIR pipeline are alternately optimized until the ranking performance converges. 
Specifically, we use the pairwise learning-to-rank loss to train the neural retrieval models during both the pretraining and fine-tuning stage: 
\begin{equation}
	\label{rank_loss}
\mathcal{L}_{rank} = \max (0, 1 - f(q, d^+)  + f(q, d^-) )
\end{equation}

where $d^+$ is a document that is more relevant to the query $q$ than the document $d^-$.



==> sections/preliminary.tex <==
% !TEX root =  ../cikm2020-fp-xiangsheng.tex

\section{Preliminaries}
\label{preliminart}
We aim to use graph information to build representations of queries and documents so as to  improve basic ranking models that only exploit textual information. 
In this section, we give the notation and introduce the basic ranking models used in our framework. 

\subsection{Notation}
Let $\mathcal{G} = (V , E)$ be an undirected graph consisting of a set of nodes $V$ and a set of edges $E$. 
We focus on two graphs: the session-flow graph and the click-through bipartite graph, where $V$ consists of queries $q \in Q$ and documents $d \in D$. 
The set $E$ contains two kinds of edges $q\to q$ and $q\to d$, which represent consecutive queries in the same session and documents clicked following a query. 
Given a node with its text content $u = \{w_1,\ldots,w_{u}\} \in V$, we write $\mathcal{N}(u)$ for its neighborhood, i.e., the set of nodes connected to it. 
The graph $\mathcal{G}$ is generated from user behaviors on the training set. 
Given a query $q$, document $d$, and graph $\mathcal{G}$, the goal of our models is to estimate the relevance of $d$ by generating high-quality representations that preserve both structural proximity information in the graph and semantic information in content. 

\subsection{Basic ranking models}
\label{text_encoder}
We focus on enriching learned representations with graph information. 
Therefore, we build on representation-based ranking models as the basic ranking models instead of interaction-based ranking models since interaction-based models do not learn an independent representation for a specific query or document.
The basic ranking model includes two parts: a text encoder and an output layer. 
To fairly compare the effectiveness of different text encoders, we apply the same output layer to predict relevance.
Depending on the specific situations in practical systems, the basic ranking model could be any representation-based ranking models.
In our work, we adopt three representation-based models as our basic ranking models, i.e., ARCI~\cite{hu2014convolutional}, DSSM~\cite{huang2013learning} and Transformer~\cite{vaswani2017attention}.

\subsubsection{ARCI} 
Given the textual content of a query or document, ARCI takes as input the embedding of its words and summarizes the meaning of that content through a layer of convolutions and pooling, until reaching a fixed length representation in the final layer.
We write $\textbf{x}_i \in \mathbb{R}^L$ to denote the word embedding with $L$ dimensions. 
An $n$-gram in the text content is represented as the concatenation of words $\textbf{x}_{i:j} =[\textbf{x}_i\oplus \textbf{x}_{i+1}\oplus \dots \oplus \textbf{x}_j]$. The final text representation is computed as follows:

\vspace{-3mm}
\begin{align}
c_{k,i} & = f(\textbf{w}_k^T \textbf{x}_{i:i+h-1} + b_k) \nonumber \\
\hat{c}_k & = \max\{c_{k,1},c_{k,2},\dots,c_{k,n-h+1}\} 
\label{cnn} \\
\textbf{c} & = [\hat{c}_1 \oplus \hat{c}_2 \oplus \cdots \oplus \hat{c}_K],
\nonumber 
\end{align}

\vspace{-1.5mm}\noindent%
where $K$ is the number of convolution kernels, $\textbf{w}_k \in \mathbb{R}^{hL}$ and $b_k \in \mathbb{R}$ are the weights in the $k$-th convolution kernel, extracting a window of $h$ words to produce a local feature. 
Also, $f$ is an activation function such as the ReLU. 
Then, the most important feature over all positions is captured by the max-pooling function. 
The features of different kernels are concatenated as the final text representation, denoted as $\textbf{c}$.

\subsubsection{DSSM} 
The first layer of the original DSSM model is a word-hashing layer, which transforms the high-dimensional term vector of the query/document to a low-dimensional letter-trigram vector.
However, this layer is not applicable to our Chinese dataset since a Chinese sentence is composed of single words, not fine-grained letters.
To address this problem, we replace the word-hashing layer as an Average Word Embedding (AWE) layer~\citep{zamani2016estimating}, which induces text embedding by averaging the embedding vectors of all terms. 
AWE has been shown to be effective in previous studies~\citep{zamani2016estimating} and is able to learn good text representation.

In summary, in our framework DSSM first averages the word embedding of all terms in the text content, and then it applies multi-layer neural networks to map text features to a semantic representation. 
The final text representation is computed as follows:
%
\begin{equation}
\label{dnn}
\begin{aligned}
\hat{\textbf{x}}_0 & = \tanh \left(W_0 \cdot \frac{\sum_{i}\textbf{x}_i}{T} + b_0\right) \\
\hat{\textbf{x}}_j & = \tanh \left(W_j \cdot \hat{\textbf{x}}_{j-1} + b_j\right), j = 1,\dots, J,
\end{aligned}
\end{equation}
%
where $T$ is the text length and $J$ is the number of hidden layers. The final $\hat{\textbf{x}}_J$ is considered as the text representation. 

\subsubsection{Transformer} 
The Transformer~\cite{vaswani2017attention} is a seq2seq model that relies on (self-)attention and several identical layer stacks.
Each layer is composed of a multi-head self-attention mechanism and  a position-wise fully connected feed-forward network.
Multi-headed attention builds multiple ``representation subspaces'' and heads governed by separate sets of $W_Q ,W_K ,W_V$ weight matrices, which are calculated as follows:   
%
%\vspace{-2mm}
 \begin{equation}
 \label{trans_eq}
 \begin{aligned}
\mathit{head}_i & = \text{Attention}(HW_Q^i,HW_K^i,HW_V^i) \\
\text{Attention}(Q,K,V) & =\text{softmax}\left(\frac{QK^T}{\sqrt{d_k}}\right)V,
 \end{aligned}
 \end{equation}
% 
 where $H$ is an embedding matrix for the bottom encoder, i.e., query or document embedding matrix. We use this stack of $N $ Transformer blocks and the output embedding of the last block is considered as the query or document representation. 

\subsubsection{Output layer}
We use the above methods to build a query representation $\textbf{e}_q$ and document representation $\textbf{e}_d$, separately. 
To fairly compare the quality of learned representations, we use the same relevance scoring function $s(q,d)$ for all basic models, which is a linear transformation for the concatenation of $\textbf{e}_q$ and $\textbf{e}_d$:
%
\begin{equation}
\label{scoring}
s(q,d) = W_s \cdot [\textbf{e}_q, \textbf{e}_d] + b_s.
\end{equation}
%
The ranking loss $\mathcal{L}_{rank}$ is defined as a pairwise ranking loss: document $d^+$ is ranked higher than $d^-$ in terms of ground truth preferences, with respect to a query $q$; 
%
\begin{align}
	\mathcal{L}_{rank} & = \max(0,1-s(q,d^+)+s(q,d^-)).
	\label{rank_loss}
\end{align}



==> sections/related_work.tex <==
% !TEX root =  ../wsdm2022-fp-xiangsheng.tex

%\vspace{-1mm}
\section{Related work}
\label{related work}
%\subsection{Query reformulation}
%Compared with traditional IR models like BM25 and learning to rank (L2R) approaches that learn over a set of hand-crafted features, neural retrieval models typically learn semantic representations from the raw text of a query and document~\cite{pang2017deep}.
%Neural methods tend to be data-hungry and requires more training data to obtain a good ranking performance~\cite{mitra2017neural}.
%A bottleneck in information retrieval is short queries 
Query reformulation is categorized into query expansion (or query anchoring) and query rewriting. 
The former aims to select and add terms to the original query while the latter is detailed rephrase of the original query with seq-to-seq model~\cite{he2016learning}.
In our work, we focus on query expansion with the goal of minimizing query-document mismatch.
The term mismatch problem is mainly caused by polysemy (same words with different meanings, e.g., Apple) and synonymy (different words with the same or similar meanings, e.g., USA and America). 
Early work investigated a range of seminal techniques such as vector feedback~\cite{rocchio1971relevance},  co‐occurrent terms~\cite{harper1978evaluation} and comparative analysis of term distributions~\cite{doszkocs1978aid}. 
%However, these potential relevant terms are not enough to expand a good query to represent users' information needs. 
To enlarge the vocabulary correlated with the query terms, a variety of data sources are employed to improve the quality of reformulated queries, such as synonyms dictionary~\cite{miller1995wordnet} and top retrieved documents~\cite{xu2017quary}.
The latter is also called pseudo relevance feedback (PRF), which is popularly exploited in different fields to improve the query representation~\cite{yang2018response,zamani2016pseudo}.
Some studies~\cite{yang2018response} only simply take all the PRF terms as side information to improve the query representation.
To select terms with better quality, different strategies to estimate the relevance of PRF terms were proposed, such as using probability language model~\cite{croft2001relevance}, supervised classification methods~\cite{cao2008selecting}  and reinforcement learning technique~\cite{nogueira2017task}.
However, these methods are mostly built on a unsupervised ranking model (e.g., BM25). 
The cooperative optimization between automatic query reformulation and neural retrieval models remain to be investigated.

On the other hand, short and ambiguous queries are the bottleneck of information retrieval, which are often vague to represent users' information needs~\cite{mitra2017neural} and limit the ranking performance of most neural retrieval models. 
Previous works on few shot retrieval~\cite{yu2021few} and weak supervision~\cite{zhang2020selective} enlarge the training corpus and learn a more robust retrieval model. 
Different from these methods, our pipeline directly learns from the original corpus and does not incorporate weak supervised signals into the training process.













%Since the majority of web search queries are short~\cite{brandao2014learning}, understanding users' search intent underlying a query becomes increasingly important for an improved search experience.
%A critical problem to understand users' search intent is the term mismatch problem, where the indexers and the users often use different words to express the same or similar meanings~\cite{carpineto2012survey}. 

%To address this mismatch problem, query reformulation technique is proposed to automatically alter a given query to other alternative queries that better represents users' information needs. 
%Early work investigated a range of seminal techniques such as vector feedback~\cite{rocchio1971relevance},  co‐occurrent terms~\cite{harper1978evaluation} and comparative analysis of term distributions~\cite{doszkocs1978aid}. 
%However, these potential relevant terms are not enough to expand a good query to represent users' information needs. 
%To enlarge the vocabulary correlated with the query terms, a variety of data sources are employed to improve the quality of reformulated queries, such as synonyms dictionary~\cite{miller1995wordnet} and top retrieved documents~\cite{xu2017quary}.
%The latter is also called pseudo relevance feedback (PRF), which is popularly exploited in different fields to improve the query representation~\cite{yang2018response,zamani2016pseudo}.
%Some studies~\cite{yang2018response} only simply take all the PRF terms as side information to improve the query representation.
%To select terms with better quality, different strategies to estimate the relevance of PRF terms were proposed, such as using probability language model~\cite{croft2001relevance} and supervised classification methods~\cite{cao2008selecting}.
%%Croft et al.~\cite{croft2001relevance} applied probability language model to estimate the relevance of each PRF term and picked up the most relevant terms to reformulate a query.
%%Cao et al.~\cite{cao2008selecting} considered PRF terms selection procedure as a supervised classification problem. 
%However, these methods suffered from some problems such as limited retrieval improvements and costly labeling expense.
%To improve the retrieval performance of the reformulated query, Rodrigo et al.~\cite{nogueira2017task} exploited reinforcement learning to select PRF terms.
%Among different strategies, reinforcement learning technique is shown better effectiveness 
%in various IR problems with non-differentiable metrics through policy gradient~\cite{nogueira2017task,montazeralghaem2020reinforcement}.
%
%
%%in selecting relevant PRF terms and obtains better retrieval performance~\cite{nogueira2017task,montazeralghaem2020reinforcement}.
%%Reinforcement learning provides a more effective way to guide the selection and obtain better retrieval performance without requiring explicitly labeled signals.
%However, these methods do not exploit external knowledge to reformulate queries, thus cannot reasonably infer the relevant terms beyond the pseudo relevance feedback. 
%If the issued query is misinterpreted by the search engine, PRF terms are mostly invalid. 
%Knowledge information has been shown effectiveness for improving query reformulation in previous studies~\cite{dalton2014entity,brandao2014learning,xiong2015query}.
%However, these methods cannot be optimized with non-differentiable ranking metrics and are limited in probabilistic relevance models (BM25).
%We extend their approaches using reinforcement learning to better select candidate terms and empower neural retrieval models in query reformulation framework.
%In addition, we conduct detailed analysis on how knowledge information can be well exploited in query reformulation, thereby providing a guidance for incorporating external knowledge for automatic query reformulation.
%
%
%
% 
%
%
%
%
%
%
%

